The physical drivers of the atomic hydrogen-halo mass relation

We use SHARK, a semi-analytic galaxy formation model, to investigate the physical processes involved in dictating the shape, scatter and evolution of the HI-halo mass relation at $0\leq z \leq 2$. We compare SHARK with HI clustering and spectral stacking of the HI-halo mass relation derived from observations finding excellent agreement with the former and a deficiency of HI in SHARK at $M_{\rm vir}\approx 10^{12-13} M_{\odot}$ in the latter, but otherwise great agreement below and above that mass threshold. In SHARK, we find that the HI mass increases with the halo mass up to a critical mass of $\approx 10^{11.8} M_{\odot}$; between $\sim 10^{11.8}-10^{13}M_{\odot}$, the scatter in the relation increases by 0.7 dex and the HI mass decreases with the halo mass on average; at $M_{\rm vir} \geq 10^{13} M_{\odot}$, the HI content continues to increase with halo mass. We find that the critical halo mass of $\approx 10^{12} M_{\odot}$ is largely set by feedback from Active Galactic Nuclei (AGN), and the exact shape and scatter of the HI-halo mass relation around that mass is extremely sensitive to how AGN feedback is modelled, with other physical processes playing a less significant role. We determine the main secondary parameters responsible for the scatter of the HI-halo mass relation, namely the halo spin parameter at $M_{\rm vir}\leq 10^{11.8} M_{\odot}$, and the fractional contribution from substructure to the total halo mass for $M_{\rm vir}\geq 10^{13} M_{\odot}$. The scatter at $10^{11.8}<M_{\rm vir}<10^{13} M_{\odot}$ is best described by the black-hole-to-stellar mass ratio of the central galaxy, reflecting the AGN feedback relevance. We present a numerical model to populate dark matter-only simulations with HI at $0\leq z \leq 2$ based solely on halo parameters that are measurable in such simulations.

==> discarded.tex <==
% -------------------------------------------------------------------------------------------------------------------------
%%%%  Developing H\,{\textsc i}--halo - Satellite density distribution %%%%%%%%
% -------------------------------------------------------------------------------------------------------------------------

% #########################################################################################################################################

\begin{figure*}
  \includegraphics[width=0.8\linewidth]{Figures/satellite_distribution_schechter.png}
\caption{The $z=0$  \hi\ distribution in the satellites of haloes with different virial mass, as labelled {\bf (virial masses are presented in the plots in units of $M_{\odot}$)}. Each distribution can be fitted with a Gamma distribution (dashed curves) as described in Equation~\ref{eq:gamma}. It is noticeable that as we move from lower to higher virial masses, the peak of the distribution shifts more towards lower \hi\ masses.}
\label{fig:satellite-density}
 \end{figure*}
 

% #########################################################################################################################################


\subsection{\hi\ Distribution in Satellite Galaxies}
\label{subsec:HI_satellite_distribution}


We know from previous figures (see Figs~\ref{fig:age_50} to \ref{fig:BH-mstar}) that for $M_{\rm vir} \gtrsim 10^{12.5}\,{\rm M}_{\odot}$, most of the \hi\ in halos resides in the satellite galaxy population (as opposed to the central). %Since we have the total \hi\ content of haloes information along with the substructure information, we wanted to see if we could use it to predict the \hi\ mass distribution in the satellites of a halo.  
We go one step beyond fitting for the summed \hi\ content of satellites in these high-mass haloes, and fit the \emph{distribution} of satellites' \hi\ masses for a given halo. This is useful as in massive halos, mock observations may require to populate individual subhalos with realistic \hi~masses.

Of the common analytic probability distribution functions that we tested, we find that the \hi\ mass distribution in satellites most resembles a \textit{Schechter}~distribution, which is defined as
%
\begin{equation}
    y \equiv log_{\rm 10}(\phi^{\star}) + \alpha(log_{\rm 10}(M) - log_{\rm 10}(M_{\star})) - \frac{log_{10}(e)}{L^{\star}}10^{M}  
    \label{eq:gamma}
\end{equation}
%
where $x \in (0,\infty)$ and $k$ is taken as the shape parameter for the Gamma function $\Gamma(k)$, with $\theta$ being the scale parameter for the fit. In Figure~\ref{fig:satellite-density}, we show the gamma fit for the $z=0$ satellite's \hi\ mass distribution for different halo-mass bins. As we move from $10^{12.6}\,{\rm M}_{\odot} < M_{\rm vir} \leq 10^{15}\,{\rm M}_{\odot}$, we find an increase in the number of satellites, leading to a smoother distribution. The true distributions in the figure are normalised histograms for the number of satellites as a function of their \hi~mass. The dashed line is the gamma fit to each distribution. The values for the fitted parameters used are tabulated in the Appendix~\ref{appendix:Spline-Fits}.



==> wordcount.tex <==


\begin{abstract}

We use the state-of-the-art semi-analytic galaxy formation model, \shark, to investigate the physical processes involved in dictating the shape, scatter and evolution of the \hi--halo mass relation at $0 \leq z \leq 2$. We compare \shark\ with \hi~clustering and spectral stacking of the \hi--halo mass relation derived from observations finding excellent agreement with the former and a deficiency of \hi\ in \shark\ at $M_{\rm halo}\approx$ \solarValue{12-13} in the latter, but otherwise great agreement below and above that mass threshold. In \shark, we find that the \hi\ mass increases with the halo mass up to a critical mass of $\approx$ \solarValue{11.8}; between $\approx$ \solarValue{11.8} and \solarValue{13}, the scatter in the relation increases by $0.7$~dex and the \hi\ mass decreases with the halo mass on average (till $M_{\rm halo}\sim 10^{12.5}\,\rm M_{\odot}$, after which it starts increasing); at $M_{\rm halo}\gtrsim 10^{13}\,\rm M_{\odot}$, the \hi\ content continues to increase with increasing halo mass, as a result of the increasing \hi\ contribution from satellite galaxies. We find that the critical halo mass of $\approx$ \solarValue{12} is largely set by feedback from Active Galactic Nuclei (AGN), and the exact shape and scatter of the \hi--halo mass relation around that mass is extremely sensitive to how AGN feedback is modelled, with other physical processes (e.g. stellar feedback, star formation and gas stripping in satellites) playing a less significant role. We also determine the main secondary parameters responsible for the scatter of the \hi--halo mass relation, namely the halo spin parameter at \subsuperscript{M}{vir}{} $<$ \solarValue{11.8}, and the fractional contribution from substructure to the total halo mass (\fracmvir) for \subsuperscript{M}{vir}{} $>$ \solarValue{13}. The scatter at \solarValue{11.8} $<$ \subsuperscript{M}{vir}{} $<$ \solarValue{13} is best described by the black-hole-to-stellar mass ratio of the central galaxy, reflecting the relevance of AGN feedback. We present a numerical model to populate dark matter-only simulations with \hi\ at $0\le z\le 2$ based solely on halo parameters that are measurable in such simulations. 
\end{abstract}

